The Space of Interaction (long version)

The space complexity of functional programs is not well understood. In particular, traditional implementation techniques are tailored to time efficiency, and space efficiency induces time inefficiencies, as it prefers re-computing to saving. Girard's geometry of interaction underlies an alternative approach based on the interaction abstract machine (IAM), claimed as space efficient in the literature. It has also been conjectured to provide a reasonable notion of space for the lambda-calculus, but such an important result seems to be elusive. In this paper we introduce a new intersection type system precisely measuring the space consumption of the IAM on the typed term. Intersection types have been repeatedly used to measure time, which they achieve by dropping idempotency, turning intersections into multisets. Here we show that the space consumption of the IAM is connected to a further structural modification, turning multisets into trees. Tree intersection types lead to a finer understanding of some space complexity results from the literature. They also shed new light on the conjecture about reasonable space: we show that the usual way of encoding Turing machines into the lambda calculus cannot be used to prove that the space of the IAM is a reasonable cost model.

==> latex-macros/ben-macros-nets.tex <==
%% tikz
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{backgrounds}
\usetikzlibrary{decorations.shapes}
\usetikzlibrary{decorations.text}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{matrix}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows}
\usetikzlibrary{positioning}
\usepackage[nofancy]{tikz-inet}

\setboolean{withimages}{true}

\tikzset{%
%
% tikzpictures
  ocenter/.style={baseline={([yshift=-.5ex, xshift=-.5ex]current bounding box)}},  
%
% NODE STYLES
  nospace/.style={inner sep= 0pt},
  etic/.style={inner sep= 0.5pt, fill=white, anchor= center},
  letic/.style={inner sep= 0.7pt, fill=white, anchor= center,circle,draw=black},
%
% MELL nets  
  port/.style={inner sep= 0.3pt, anchor= center,circle,draw=black,fill=black, minimum size = 0.3pt},
%
% cbv nets  
  eport/.style={inner sep= 0.8pt, anchor= center,circle,draw=cyan,fill=white, minimum size = 0.8pt},
  mport/.style={inner sep= 0.8pt, anchor= center, circle,draw=white,fill=brown, minimum size = 0.8pt, solid, 
line width=0.10ex},
% cbn nets  
  eportn/.style={inner sep= 0.8pt, anchor= center,circle,draw=blue,fill=white, minimum size = 0.8pt},
  mportn/.style={inner sep= 0.8pt, anchor= center, circle,draw=red,fill=red, minimum size = 0.8pt, solid, 
line width=0.10ex},
%
%
% EDGE STYLES
  nopol/.style={->, shorten <=0.5pt, shorten >=0.5pt, draw=gray, line width=0.18ex},
  nopolrev/.style={<-, shorten <=1pt, shorten >=1pt, draw=gray, line width=0.18ex},
  nopolgen/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=gray,-](0pt,3pt) -- (0pt,-3pt);}},->, shorten <=0.5pt, shorten >=0.5pt, draw=gray, line width=0.18ex},
  nopolrevgen/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=gray,-](0pt,3pt) -- (0pt,-3pt);}},<-, shorten <=1pt, shorten >=1pt, draw=gray, line width=0.18ex},
  outEdge/.style={<-, shorten >=0.5pt, shorten <=0.5pt, draw=blue, line width=0.18ex},
  inpEdge/.style={->, densely dotted, shorten >=0.5pt, shorten <=0.5pt, draw=red, line width=0.18ex, overlay},
  inpEdgeGen/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=red,-](0pt,3pt) -- (0pt,-3pt);}},->, densely dotted, shorten >=0.5pt, shorten <=0.5pt, draw=red, line width=0.18ex, overlay},
  %
  % cbv nets
    eprinc/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.5pt, anchor= center,circle,draw=cyan, fill=cyan, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprinc/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.5pt, anchor= center,circle,draw=brown, fill=brown, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprincpar/.style={postaction={decorate},decoration={markings,mark=at position .6 with {\node [inner sep= 0.5pt, anchor= center,circle,draw=brown, fill=brown, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    pure/.style={->, shorten <=1pt, shorten >=1pt, draw=brown, line width=0.18ex},
    pureRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=brown, line width=0.18ex},
    exppure/.style={->, shorten <=1pt, shorten >=1pt, draw=cyan, line width=0.18ex, densely dotted},
    exppureRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=cyan, line width=0.18ex, densely dotted},    genexppure/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=cyan,-](0pt,3pt) -- (0pt,-3pt);}},->, shorten <=1pt, shorten >=1pt, draw=cyan, line width=0.18ex, densely dotted},
    enaryedge/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=cyan,-](0pt,3pt) -- (0pt,-3pt);}}},
  % cbn nets
    eprincn/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.7pt, anchor= center,circle,draw=blue, fill=blue, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprincn/.style={postaction={decorate},decoration={markings,mark=at position .6 with {\node [inner sep= 0.7pt, anchor= center,circle,draw=red, fill=white, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprincnpar/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.7pt, anchor= center,circle,draw=red, fill=white, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    puren/.style={->, shorten <=1pt, shorten >=1pt, draw=red, line width=0.18ex},
    purenRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=red, line width=0.18ex},
    exppuren/.style={->, shorten <=1pt, shorten >=1pt, draw=blue, line width=0.18ex, densely dotted},
    exppurenRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=blue, line width=0.18ex, densely dotted},    genexppuren/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=blue,-](0pt,3pt) -- (0pt,-3pt);}},->, shorten <=1pt, shorten >=1pt, draw=blue, line width=0.18ex, densely dotted},
    enaryedge/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=blue,-](0pt,3pt) -- (0pt,-3pt);}}},
%
% BOX LINE STYLES
  jboxline/.style={draw= gray,rounded corners, line width=0.20ex, overlay},
  exboxline/.style={draw= gray,line width=0.20ex, overlay},
  noboxline/.style={draw= white,rounded corners, line width=0ex},
%
% NETS
  net/.style={draw=gray,inner sep=2pt,thick,ellipse, anchor=center, font=\scriptsize},
  inductiveTr/.style={draw=black!50, minimum size=0.9cm},
  inductiveTrSmall/.style={draw=black!50, minimum size=0.6cm},
%
% EVERY
  every label/.style={label distance = 1pt, font=\scriptsize, inner sep= 1pt},  
  every node/.style={font=\scriptsize }%\small
}
%\node[etic,fill=white]{{\tiny 0}}

\newcommand{\altax}{8pt}
\newcommand{\altcut}{8pt}


\newcommand{\staltb}{30pt}
\newcommand{\stlarb}{25pt}
\newcommand{\hstaltb}{\staltb/2}
\newcommand{\hstlarb}{\stlarb/2}

\newcommand{\stalt}{22pt}
\newcommand{\stlar}{15pt}
\newcommand{\hstalt}{\stalt/2}
\newcommand{\hstlar}{\stlar/2}
\newcommand{\hhstalt}{\stalt/4}
\newcommand{\hhstlar}{\stlar/4}

\newcommand{\staltm}{17.8pt}
\newcommand{\stlarm}{13.6pt}
\newcommand{\hstaltm}{\staltm/2}
\newcommand{\hstlarm}{\stlarm/2}

\newcommand{\ilar}{12pt}
\newcommand{\hilar}{\ilar/2}

\newcommand{\auxdistance}{5pt}
\newcommand{\pendingdist}{10pt}
\newcommand{\anchorh}{9pt}
\newcommand{\anchorw}{9pt}

%LINKS
\input{\macrospath/graphical-macros/generic-links}
\input{\macrospath/graphical-macros/links-MELL}

%SEPARATORI
\newcommand{\invsep}[2]{%parametri: #1=larghezza della separazione,
                                                   %#2= altezza del separatore
  \begin{tikzpicture}[ocenter]%separatore
    \node (up){};
    \node at (up.center) [below right=#2 and #1](down){};
  \end{tikzpicture}
}

\newcommand{\sepColonne}[2]{%parametri: #1=larghezza della separazione,
                                                   %#2= altezza del separatore
  \begin{tikzpicture}[ocenter]%separatore
    \node (up){};
    \node at (up) [below=#2](down){};
    \draw [color=gray] (up) to (down);
    \node at (up) [left = #1] (left){};
    \node at (up) [right= #1] (right){};
  \end{tikzpicture}
}

\newcommand{\sepRows}[2]{%parametri: #1=Larghezza della separazione,
                                                   %#2= altezza del separatore
  \begin{tikzpicture}[ocenter]%separatore
    \node (up){};
    \node at (up) [right=#1](down){};
    \draw [color=gray] (up) to (down);
    \node at (up) [above = #2] (left){};
    \node at (up) [below= #2] (right){};
  \end{tikzpicture}
}

\newcommand{\lineasep}{\multicolumn{6}{c}{\sepRows{200pt}{0.5pt}}}
\newcommand{\lineaseplong}{\multicolumn{9}{c}{\sepRows{350pt}{0.5pt}}}

\newcommand{\gdots}[3]{
% 1 = left node
% 2 = right node
% 3 = eventual parameters
\node at ($(#1)!.5!(#2)$) [#3]{\tiny $\ldots$};
}

\newcommand{\gdotsname}[4]{
% 1 = left node
% 2 = right node
% 3 = eventual parameters
% 4 = name of the node
\node at ($(#1)!.5!(#2)$) [#3](#4){\tiny $\ldots$};
}

\newcommand{\bracketup}[5]{
% 1 = left node
% 2 = right node
% 3 = height
% 4 = label
% 5 = name
\node at \med{#1}{#2}[above=#3, nospace](#4){};

\draw[out=90, in=-90] (#1) to (#4);
\draw[out=90, in=-90] (#2) to (#4);
\node at (#4.center)[ above=\sepbox, nospace](#4label){#5};
}

\newcommand{\bracketdown}[5]{
% 1 = left node
% 2 = right node
% 3 = height
% 4 = label
% 5 = name
\node at \med{#1}{#2}[below=#3, nospace](#4){};

\draw[out=-90, in=90] (#1) to (#4);
\draw[out=-90, in=90] (#2) to (#4);
\node at (#4.center)[ below=\sepbox, nospace](#4label){#5};}

\newcommand{\mednop}[2]{
$(#1)!.5!(#2)$
}

==> latex-macros/graphical-macros/generic-links.tex <==
%%%%%%%%%%%%%%%%
%% AXIOM
%%%%%%%%%%%%%%%

\newcommand{\axnode}[5]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = height
% 5 = label size
\node at ($(#1.center)!.5!(#2.center)$) [above = #4, etic] (#3){ #5$\ax$};}

\newcommand{\axedges}[5 ]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = left edge line style
% 5 = right edge line style
\draw[#4, in=90, out=180] (#3) to (#1);
\draw[#5, in=90, out=0] (#3) to (#2);
}

\newcommand{\laxabstract}[7]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = height
% 5 = label size
% 6 = left edge line style
% 7 = right edge line style
\axnode{#1}{#2}{#3}{#4}{#5}
\axedges{#1}{#2}{#3}{#6}{#7}
}

%%%%%%%%%%%%%%%%
%% CUT
%%%%%%%%%%%%%%%

\newcommand{\cutnode}[5]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = height
% 5 = label size
\node at ($(#1.center)!.5!(#2.center)$) [below = #4, etic] (#3){ #5$\cut$};}

\newcommand{\cutedges}[5 ]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = left edge line style
% 5 = right edge line style
\draw[#4, out=-90, in=180] (#1) to (#3);
\draw[#5, out=-90, in=0] (#2) to (#3);
}

\newcommand{\lcutabstract}[7]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = height
% 5 = label size
% 6 = left edge line style
% 7 = right edge line style
\cutnode{#1}{#2}{#3}{#4}{#5}
\cutedges{#1}{#2}{#3}{#6}{#7}
}


%%%%%%%%%%%%%%%%
%% ZERARY
%%%%%%%%%%%%%%%

\newcommand{\lZeroary}[5]{
% 1 = one principal port	
% 2 = name of the link
% 3 = link symbol
% 4 = distance link-node
% 5 = type of edge
\node at (#1.center) [above= #4, etic] (#2){#3};
\draw[#5] (#2) to (#1);}


%%%%%%%%%%%%%%%%
%% UNARY
%%%%%%%%%%%%%%%

\newcommand{\lUnarySymbol}[5]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link, 
% 4 = link symbol
% 5 = node style
\node at ($(#2.center) ! .5 ! (#1.center)$) [#5] (#3){ #4};
}

\newcommand{\lUnary}[5]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
% 4 = link symbol
% 5 = edge line
\lUnarySymbol{#1}{#2}{#3}{#4}{etic}

\draw[#5] (#2) to (#3);
\draw[#5] (#3) to (#1);
}

\newcommand{\lUnaryDiffEdges}[6]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
% 4 = link symbol
% 5 = bottom edge line
% 6 = top edge line 

% symbol
\lUnarySymbol{#1}{#2}{#3}{#4}{etic}

% bottom edge
\draw[#5] (#3) to (#1);

%above edge
\draw[#6] (#2) to (#3);
}

\newcommand{\lUnaryDiffEdgesCircle}[6]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
% 4 = link symbol
% 5 = bottom edge line
% 6 = top edge line 

% symbol
\lUnarySymbol{#1}{#2}{#3}{#4}{letic}

% bottom edge
\draw[#5] (#3) to (#1);

%above edge
\draw[#6] (#2) to (#3);
}

\newcommand{\lUnaryDiffEdgesCircleNode}[7]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
% 4 = link symbol
% 5 = bottom edge line
% 6 = top edge line 
% 7 = node parameters

% symbol
\lUnarySymbol{#1}{#2}{#3}{#4}{#7}

% bottom edge
\draw[#5] (#3) to (#1);

%above edge
\draw[#6] (#2) to (#3);
}


%%%%%%%%%%%%%%%%
%% BINARY
%%%%%%%%%%%%%%%

\newcommand{\lBinSymbol}[6]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = node style
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [#6] (#4){#5};
}

\newcommand{\lBinSymbolFixR}[6]{
% parameters
% 1 =  principal port,
% 2 = left auxiliary port,
% 3 = right auxiliary port,
% 4 = name of the link, 
% 5 = link symbol
% 6 = node style
\node at ($(#1.center) ! .5 ! (#3 -| #1)$) [below= 1pt, #6] (#4){#5};
}

\newcommand{\lBinSymbolFixL}[6]{
% parameters
% 1 =  principal port,
% 2 = left auxiliary port,
% 3 = right auxiliary port,
% 4 = name of the link, 
% 5 = link symbol
% 6 = node style
\node at ($(#1.center) ! .5 ! (#3 -| #2)$) [below= 1pt, #6] (#4){#5};
}


\newcommand{\lBinEdgesAbove}[5]{
% 1 = left auxiliary port	
% 2 = right auxiliary port	
% 3 = name of the link
% 4 = left edge type
% 5 = right edge type
\draw[#4, in=150, out=-90] (#1) to (#3);
\draw[#5, in=30, out=-90] (#2) to (#3);
}

\newcommand{\lBinEdgesBelow}[5]{
% 1 = left auxiliary port	
% 2 = right auxiliary port	
% 3 = name of the link
% 4 = left edge type
% 5 = right edge type
\draw[#4, in=210, out=90] (#1) to (#3);
\draw[#5, in=-30, out=90] (#2) to (#3);
}


\newcommand{\lBinaryWithEdgeAboveTypes}[8]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = principal edge type
% 7 = left premise edge type
% 8 = right premise edge type
\lBinSymbol{#1}{#2}{#3}{#4}{#5}{etic}

% upper edges of the link
\lBinEdgesAbove{#2}{#3}{#4}{#7}{#8}

\draw[#6] (#4) to (#1);
}

\newcommand{\lBinaryWithEdgeBelowTypes}[9]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = principal edge type
% 7 = left premise edge type
% 8 = right premise edge type
% 9 = node style
\lBinSymbol{#1}{#2}{#3}{#4}{#5}{#9}

% upper edges of the link
\lBinEdgesBelow{#2}{#3}{#4}{#7}{#8}

\draw[#6] (#4) to (#1);
}


\newcommand{\lBinary}[6]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = edge type
\lBinaryWithEdgeAboveTypes{#1}{#2}{#3}{#4}{#5}{#6}{#6}{#6}
}

\newcommand{\lBinaryFlipped}[6]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = edge type
\lBinaryWithEdgeBelowTypes{#1}{#2}{#3}{#4}{#5}{#6}{#6}{#6}{etic}
}


%%%%%%%%%%%%%%%%
%% BOXES
%%%%%%%%%%%%%%%

\newcommand{\stboxlw}{6pt}
\newcommand{\stboxh}{20pt}
\newcommand{\stboxrw}{30pt}
\newcommand{\stboxrwaux}{35pt}
\newcommand{\sepbox}{2pt}
\newcommand{\belowbox}{\stboxh+2*\sepbox+1pt}

\newcommand{\boxnodes}[4]{
% 1 = link to box
% 2 = left width
% 3 = right width 
% 4 = height
\node at (#1.center)[left = #2,nospace](#1so){};
\node at (#1.center)[right = #3,nospace](#1se){};
\node at (#1se.center)[above=#4,nospace](#1ne){};
\node at (#1ne-|#1so)[nospace](#1no){};}

\newcommand{\BoxNodesWithPalOnTopAndVeticalNodeBound}[4]{
% 1 = upper node (pal of ! link) 
% 2 = bottom node 
% 3 = box left width
% 4 = box right width
\node at (#1.center)[left = #3,nospace](#1no){};
\node at (#1.center)[right = #4,nospace](#1ne){};
\node at (#1no|-#2)[nospace](#1so){};
\node at (#1ne|-#2)[nospace](#1se){};
}


\newcommand{\boxline}[2]{
% 1 = box link
% 2 = line style
\draw[#2](#1.center) -- (#1se.center) -- (#1ne.center) -- (#1no.center) -- (#1so.center)--(#1.center);}

\newcommand{\BoxLineWithPalOnTop}[2]{
% 1 = box link
% 2 = line style
\draw[#2](#1so.center) -- (#1se.center) -- (#1ne.center) -- (#1.center) -- (#1no.center) -- (#1so.center); 
}

\newcommand{\abox}[5]{
% 1 = link to box
% 2 = line style
% 3 = right width 
% 4 = left width
% 5 = height
\boxnodes{#1}{#3}{#4}{#5}
\boxline{#1}{#2line}}

\newcommand{\aBoxWithPalOnTopAndVeticalNodeBound}[5]{
% 1 = upper node (pal of ! link) 
% 2 = bottom node 
% 3 = line style
% 4 = box left width
% 5 = box right width
\BoxNodesWithPalOnTopAndVeticalNodeBound{#1}{#2}{#4}{#5}
\BoxLineWithPalOnTop{#1}{#3line}
}


\newcommand{\boxauxnodes}[3]{
% 1 = link to box
% 2 = distance of the right conclusion from SE corner
% 3 = distance between the two conclusions
\node at (#1se.center)[left = #2, nospace](#1auxk){};
\node at (#1auxk.center)[left= #3, nospace](#1aux1){};
}

% \newcommand{\boxauxnodes}[2]{
% % 1 = link to box
% % 2 = box right width
% \node at (#1se.center)[left = \stboxlw, nospace](#1auxk){};
% \node at (#1auxk.center)[left= ((#2)/2), nospace](#1aux1){};
% }

\newcommand{\boxauxnodeslab}[4]{
% 1 = link to box
% 2 = left label,
% 3 = right label,
% 4 = height delta
\node at (#1auxk.center)[below = #4,etic](#1auxktarget){\tiny #3};
\node at (#1aux1.center)[below = #4,etic](#1aux1target){\tiny #2};

\draw[nopol] (#1auxk) to (#1auxktarget);
\draw[nopol] (#1aux1) to (#1aux1target);
}

\newcommand{\boxlabel}[2]{
% 1 = box link
% 2 = label
\node at ($(#1so)!.5!(#1ne)$) {#2};
}

\newcommand{\boxlineor}[3]{
% 1 = box link
% 2 = line style
% 3 = jolly point on the right
\draw[#2, overlay](#1.center) -- (#1-|#3)--(#3.center)--(#3-|#1se.center)--(#1ne.center) -- (#1no.center) -- (#1so.center)--(#1.center);}


\newcommand{\aboxor}[7]{
% 1 = link to box
% 2 = box kind
% 3 = box left width
% 4 = box right width
% 5 = box height
% 6 = label 
% 7 = jolly point
\boxnodes{#1}{#3}{#4}{#5}
\boxlineor{#1}{#2line}{#7}
\boxlabel{#1}{#6}}


%%%%%%%%%%%%%%%%
%% CONTRACTION AND WHYNOT TREES
%%%%%%%%%%%%%%%
\newcommand{\whyntreelength}{1.8*\stlar}
\newcommand{\whyntreeheigth}{1.2*\stalt}

\newcommand{\whyntreeabstract}[3]{
% 1 = principal node
% 2 = tree height
% 3 = tree base length/2
\node at (#1.center) [above left = #2 and #3, nospace](#1_left_vertex){};
\node at (#1.center) [above right = #2 and #3, nospace](#1_right_vertex){};

\draw[exboxline](#1.center) -- (#1_left_vertex.center) -- (#1_right_vertex.center) -- (#1.center);

% label
\node at (#1.center) [above=3*#2/5,nospace](#1_label){\tiny $T_{\contrp}$};

% ghost nodes for leaves
\node at (#1.center) [above left = #2 and 3*(#3/5), nospace](#1_left_group_right_node){};
\node at (#1.center) [above right = #2 and 3*(#3/5), nospace](#1_right_group_left_node){};
\node at (#1.center) [above left = #2 and #3/5, nospace](#1_center_group_left_node){};
\node at (#1.center) [above right = #2 and #3/5, nospace](#1_center_group_right_node){};
}

\newcommand{\whyntreeboxbordersabstract}[3]{
% 1 = principal node
% 2 = tree height
% 3 = tree base length/2

% boxline up right
\node at (#1_left_group_right_node.center) [below right = #2/4 and #3/10, nospace](#1_leftupboxrightnode){};
\node at (#1_leftupboxrightnode.center) [left= 2*#3/5, nospace](#1_leftupboxleftnode){};
\draw[exboxline](#1_leftupboxrightnode)to(#1_leftupboxleftnode);

% boxline left
\node at (#1_right_group_left_node.center) [below left = #2/2 and 3*#3/10, nospace](#1_rightupboxrightnode){};
\node at (#1_rightupboxrightnode.center) [right= 2*#3/5, nospace](#1_rightupboxleftnode){};
\draw[exboxline](#1_rightupboxrightnode)to(#1_rightupboxleftnode);

% boxline below right
\node at (#1.center) [above left= #2/4 and #3/20, nospace](#1_leftdownboxrightnode){};
\node at (#1_leftdownboxrightnode.center) [left= 2*#3/5, nospace](#1_leftdownboxleftnode){};
\draw[exboxline](#1_leftdownboxrightnode)to(#1_leftdownboxleftnode);

}

\newcommand{\whyntreeweakeningleavesontheleft}[1]{
% 1 = principal node
\node at (#1_left_vertex.center) [above=\hstalt, etic](#1_weak1){\tiny $\weak$};
\node at (#1_left_group_right_node.center) [above=\hstalt, etic](#1_weakn){\tiny $\weak$};

\draw[nopol](#1_weak1) to (#1_left_vertex);
\draw[nopol](#1_weakn) to (#1_left_group_right_node);

\gdots{#1_left_vertex}{#1_left_group_right_node}{above = 2pt}
}

\newcommand{\whyntreeleavesabstract}[3]{
% 1 = principal node
% 2 = tree height
% 3 = tree base length/2

% derelictions
\node at (#1_center_group_left_node.center) [above=\hstalt, etic](#1_dern){\tiny $\der$};
\node at (#1_center_group_right_node.center) [above=\hstalt, etic](#1_der1){\tiny $\der$};

\draw[nopol](#1_dern) to (#1_center_group_left_node);
\draw[nopol](#1_der1) to (#1_center_group_right_node);

\gdots{#1_center_group_left_node}{#1_center_group_right_node}{above = 2pt}

%weakening
\whyntreeweakeningleavesontheleft{#1}

% axioms
\node at (#1_right_vertex.center) [above right=\hstalt and #3/4, etic](#1_ax1){\tiny $\ax$};
\node at (#1_right_vertex.center) [right=2*#3/4, nospace](#1_ax1_ghost_concl){};
\draw[nopol, out = 180, in = 90](#1_ax1) to (#1_right_vertex);
\draw[nopol, out = 0, in = 90](#1_ax1) to (#1_ax1_ghost_concl);

\node at (#1_ax1.center) [above=3*\hstalt/4, etic](#1_axn){\tiny $\ax$};
\node at (#1_right_group_left_node.center) [right=13*#3/10, nospace](#1_axn_ghost_concl){};

\draw[nopol, out = 180, in = 90, looseness=1.8](#1_axn) to (#1_right_group_left_node);
\draw[nopol, out = 0, in = 90, looseness=1.8](#1_axn) to (#1_axn_ghost_concl);

\gdots{#1_right_vertex}{#1_right_group_left_node}{above = 2pt}

}

\newcommand{\whyntree}[1]{
% 1 = principal node
\whyntreeabstract{#1}{\whyntreeheigth}{\whyntreelength}
}

\newcommand{\whyntreeboxborders}[1]{
% 1 = principal node
\whyntreeabstract{#1}{\whyntreeheigth}{\whyntreelength}
\whyntreeboxbordersabstract{#1}{\whyntreeheigth}{\whyntreelength}
}

\newcommand{\whyntreeboxbordersleaves}[1]{
% 1 = principal node
\whyntreeboxborders{#1}{\whyntreeheigth}{\whyntreelength}
\whyntreeleavesabstract{#1}{\whyntreeheigth}{\whyntreelength}
}

\newcommand{\whyntreeboxbordersleaveswithpremises}[1]{
% 1 = principal node

\whyntreeboxbordersleaves{#1}

% dereliction premises
\node at (#1_der1.center) [above=\hstalt, nospace](#1_der1_premise){};
\node at (#1_dern.center) [above=\hstalt, nospace](#1_dern_premise){};
\draw[nopol](#1_der1_premise) to (#1_der1);
\draw[nopol](#1_dern_premise) to (#1_dern);
}

%%%%%%%%%%%%%%%%
%% BOX BORDERS
%%%%%%%%%%%%%%%
\newcommand{\boxdershorizontaldistance}{7pt}
\newcommand{\boxdersverticaldistance}{2pt}
\newcommand{\boxdersdots}{5pt}

\newcommand{\boxcornerright}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline

% internal box
\node at (#1.center)[left=#2, nospace](#1lineaso){};
\node at (#1.center)[above=#3, nospace](#1lineane){};
\draw[#4](#1lineaso.center) -- (#1.center) -- (#1lineane.center);

% internal box dotted extensions
\node at (#1lineaso.center)[left=\boxdersdots, nospace](#1lineasodotted){};
\node at (#1lineane.center)[above=\boxdersdots, nospace](#1lineanedotted){};
\draw[#4, densely dotted](#1lineaso)to(#1lineasodotted);
\draw[#4, densely dotted](#1lineane)to(#1lineanedotted);
}


\newcommand{\boxcornersright}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline
\node at (#1.center)[above right=2pt and 4pt, etic](#1dots){\tiny $...$};
\boxcornerright{#1}{#2}{#3}{#4}

% external box
\node at (#1.center)[below right=\boxdersverticaldistance and \boxdershorizontaldistance, nospace](#1linease2){};
\node at (#1lineaso.center)[below=\boxdersverticaldistance, nospace](#1lineaso2){};

\node at (#1lineane.center)[right=\boxdershorizontaldistance, nospace](#1lineane2){};
\draw[#4](#1lineaso2.center) -- (#1linease2.center) -- (#1lineane2.center);

% external box dotted extensions
\node at (#1lineaso2.center)[left=\boxdersdots, nospace](#1lineaso2dotted){};
\node at (#1lineane2.center)[above=\boxdersdots, nospace](#1lineane2dotted){};
\draw[#4, densely dotted](#1lineaso2)to(#1lineaso2dotted);
\draw[#4, densely dotted](#1lineane2)to(#1lineane2dotted);



}

\newcommand{\boxcornerleft}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline

% internal box
\node at (#1.center)[right=#2, nospace](#1lineaso){};
\node at (#1.center)[above=#3, nospace](#1lineane){};
\draw[#4](#1lineaso.center) -- (#1.center) -- (#1lineane.center);

% internal box dotted extensions
\node at (#1lineaso.center)[right=\boxdersdots, nospace](#1lineasodotted){};
\node at (#1lineane.center)[above=\boxdersdots, nospace](#1lineanedotted){};
\draw[#4, densely dotted](#1lineaso)to(#1lineasodotted);
\draw[#4, densely dotted](#1lineane)to(#1lineanedotted);
}

\newcommand{\boxcornersleft}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline

\node at (#1.center)[above left=2pt and 4pt, etic](#1dots){\tiny $...$};

\boxcornerleft{#1}{#2}{#3}{#4}

% external box
\node at (#1.center)[below left=\boxdersverticaldistance and \boxdershorizontaldistance, nospace](#1linease2){};
\node at (#1lineaso.center)[below=\boxdersverticaldistance, nospace](#1lineaso2){};

\node at (#1lineane.center)[left=\boxdershorizontaldistance, nospace](#1lineane2){};
\draw[#4](#1lineaso2.center) -- (#1linease2.center) -- (#1lineane2.center);

% external box dotted extensions
\node at (#1lineaso2.center)[right=\boxdersdots, nospace](#1lineaso2dotted){};
\node at (#1lineane2.center)[above=\boxdersdots, nospace](#1lineane2dotted){};
\draw[#4, densely dotted](#1lineaso2)to(#1lineaso2dotted);
\draw[#4, densely dotted](#1lineane2)to(#1lineane2dotted);



}


==> latex-macros/graphical-macros/links-MELL.tex <==
\newcommand{\lax}[3]{
% 1 = left port
% 2 = right port
% 3 = link name
\laxabstract{#1}{#2}{#3}{\altax}{\tiny}{nopol}{nopol}}

\newcommand{\lcut}[3]{
% 1 = left port
% 2 = right port
% 3 = link name
\lcutabstract{#1}{#2}{#3}{\altcut}{\tiny}{nopol}{nopol}}


%%%%%%%%
%% MULTIPLICATIVES
%%%%%%%%

\newcommand{\ltens}[4]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
\lBinary{#1}{#2}{#3}{#4}{$\tens$}{nopol}}

\newcommand{\lpar}[4]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
\lBinary{#1}{#2}{#3}{#4}{$\parr$}{nopol}}

\newcommand{\lone}[2]{
% 1 = one principal port	
% 2 = name of the link
\lzeroary{#1}{#2}{$\one$}{\hstalt}{nopol}}

\newcommand{\lbot}[2]{
% 1 = one principal port	
% 2 = name of the link
\lzeroary{#1}{#2}{$\bot$}{\hstalt}{nopol}}


%%%%%%%%
%% EXPONENTIALS
%%%%%%%%

\newcommand{\lder}[3]{
% parameters
% 1 = principal port	
% 2 = auxiliary port	
% 3 = name of the link
\lUnary{#1}{#2}{#3}{$\der$}{nopol}
}

\newcommand{\lbang}[3]{
% parameters
% 1 = principal port	
% 2 = auxiliary port	
% 3 = name of the link
\lUnary{#1}{#2}{#3}{$\bang$}{nopol}
}

\newcommand{\lweak}[2]{
% 1 = one principal port	
% 2 = name of the link
\lZeroary{#1}{#2}{$\weak$}{1.3*\hstalt}{nopol}
}

\newcommand{\lcontr}[4]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
\lBinary{#1}{#2}{#3}{#4}{$\contr$}{nopol}}




==> machines/KAM.tex <==
% !TeX spellcheck = en_US
% !TEX root = ../main.tex
%%%%%%%%%%%%%%
\begin{center}
	\fbox{
	$\begin{array}{c@{\hspace{1.4cm}}c@{\hspace{1.4cm}}c@{\hspace{1.4cm}}c}
	\textsc{Closures} &
	\textsc{Environments}&
	\textsc{Stacks}&
	\textsc{States}\\
	\clos  \grameq  (\tm,\ctx,\env) &  \env  \grameq  \stempty \midd \esub\var \clos\cdot \env &
	\stack  
	\grameq  \stempty \midd \clos\cdot \stack&
	\state\grameq(\tm,\ctx,\env,\stack)
	\end{array}$}\\\medskip
	${\footnotesize \begin{array}{l@{\hspace{.4cm}} 
			l@{\hspace{.4cm}}l@{\hspace{.4cm}}lll@{\hspace{.4cm}} 
			l@{\hspace{.4cm}}l@{\hspace{.4cm}}l}
		%	\newcommand{\kamstatetab}[4]{&\red{#1} && #2 && #3 && #4 }
		\mathsf{Term} & \mathsf{Ctx} & \mathsf{Env} & 
		\mathsf{Stack}
		&&	\mathsf{Term} & \mathsf{Ctx} & \mathsf{Env} 
		& 
		\mathsf{Stack}
		\\
		\hhline{=========}
		\\[-8pt]
		\kamstatetab{ \tm\tmtwo }{ \ctx }{ \stack }{ \env } &
		\kamdap &%\\[-2pt]
		\kamstatetab{ \tm }{ \ctxp{\ctxhole\tmtwo} }{ 
		(\tmtwo,\ctxp{\tm\ctxhole},\env)\cons \stack }{ \env }
		\\[3pt]				
		\kamstatetab{ \la\var\tm }{ \ctx }{ \clos\cons \stack }{ \env } &
		\kamdlam &%\\[-2pt]
		\kamstatetab{ \tm }{ \ctxp{\la\var\ctxhole} }{ \stack }{ \esub\var \clos\cons \env }
		\\[3pt]  
		\kamstatetab{ \var }{ \ctx }{ \stack }{ \env\cons\esub\var{(\tmtwo,\ctxtwo,\envthree)}\cons 
		\envtwo 
		} &
		\iamdvar &%\\[-2pt]
		\kamstatetab{ \tmtwo}{ \ctxtwo }{ 
			\stack }{ \envthree }
		\\[3pt]
		\cline{1-9}
		\end{array}}$\end{center}

